Multi-Scale Zero-Order Optimization of Smooth Functions in an RKHS

We aim to optimize a black-box function $f:\mathcal{X} \mapsto \mathbb{R}$ under the assumption that $f$ is H\"older smooth and has bounded norm in the RKHS associated with a given kernel $K$. This problem is known to have an agnostic Gaussian Process (GP) bandit interpretation in which an appropriately constructed GP surrogate model with kernel $K$ is used to obtain an upper confidence bound (UCB) algorithm. In this paper, we propose a new algorithm (\texttt{LP-GP-UCB}) where the usual GP surrogate model is augmented with Local Polynomial (LP) estimators of the H\"older smooth function $f$ to construct a multi-scale UCB guiding the search for the optimizer. We analyze this algorithm and derive high probability bounds on its simple and cumulative regret. We then prove that the elements of many common RKHS are H\"older smooth and obtain the corresponding H\"older smoothness parameters, and hence, specialize our regret bounds for several commonly used kernels. When specialized to the Squared Exponential (SE) kernel, \texttt{LP-GP-UCB} matches the optimal performance, while for the case of Mat\'ern kernels $(K_{\nu})_{\nu>0}$, it results in uniformly tighter regret bounds for all values of the smoothness parameter $\nu>0$. Most notably, for certain ranges of $\nu$, the algorithm achieves near-optimal bounds on simple and cumulative regrets, matching the algorithm-independent lower bounds up to polylog factors, and thus closing the large gap between the existing upper and lower bounds for these values of $\nu$. Additionally, our analysis provides the first explicit regret bounds, in terms of the budget $n$, for the Rational-Quadratic (RQ) and Gamma-Exponential (GE). Finally, experiments with synthetic functions as well as a CNN hyperparameter tuning task demonstrate the practical benefits of our multi-scale partitioning approach over some existing algorithms numerically.

==> Discussion.tex <==
% \vspace{-0.7em}
We discuss the improvements in the regret bounds achieved by our proposed algorithm over the existing results in Sec.~\ref{subsec:improved} and  in Sec.~\ref{subsec:practical}, we discuss some issues in efficient practical implementation of our proposed algorithm. 

%________________________________________________________________________________
% IMPROVED REGRET BOUNDS
%________________________________________________________________________________
\subsection{Improved Regret Bounds}
\label{subsec:improved}
We first summarize the regret bounds of the LP-GP-UCB algorithm:
\begin{itemize}
\item For the SE kernel, the LP-GP-UCB algorithm matches the best known bounds on both the simple and cumulative regret, which are also known to be near-optimal w.r.t. the lower bounds of \citep{scarlett2017lower}. 

\item For the case of \matern~kernels, the LP-GP-UCB algorithm with $k=0$ achieves a bound on $\creg$ of $\tOh{n^{(D+\alpha)/(D+2\alpha)}}$. While this bound is not near-optimal, it is sublinear for all values of $\nu$ and $D$ thus improving upon the results of \citep{srinivas2012information, chowdhury2017kernelized} which are linear in $n$ for $2\nu \leq D^2$. 

 For $\kmat$ with $\nu$ satisfying $2\nu<(D+1)(D+4)$ the LP-GP-UCB algorithm achieves a bound on the simple regret of $\tOh{n^{-\nu/(D + 2\nu)}}$ which matches the lower bounds of \citep{scarlett2017lower} up to poly-logarithmic factors. Thus for these values of $\nu, D$, our proposed algorithm is near-optimal in terms of simple regret. For other values of $\nu, D$ the algorithm achieves a bound of $\sreg = \tOh{n^{-\alpha/(D + 2\alpha)}}$ which, although sub-optimal, still converges to zero unlike the previous known bounds. 
 
    % \item For the case of SE and \matern~kernels, it achieves a cumulative regret of $\tOh{\igain \sqrt{n}}$ which matches the best existing bounds. Furthermore, for the case of \matern~kernels, the LP-GP-UCB algorithm with input $k=0$ and $\alpha \in \{1/2, 1\}$ also achieves a cumulative regret of $\tOh{n^{\alpha/(2\alpha+D)}}$. While this cumulative regret does not match the lower bounds of \citep{scarlett2017lower}, they are sublinear for all values of $\nu$ and $D$. 
    
    
    % \item For the \matern~kernels $\kmat$ with $\nu < (D+1)(D+4)/2$, the algorithm achieves a simple regret bound of $\sreg = \tOh{n^{-\nu/(2\nu+D)}}$ which matches the information theoretic lower bounds of \citep{scarlett2017lower}. This closes the large gap existing in literature on the simple regret bounds for these kernels. 
    \item For several other important kernels, including GE, RQ and PP, we derive the first explicit (in $n$) bounds on $\sreg$ and $\creg$ for our proposed algorithm. 
\end{itemize}


% %________________________________________________________________________________
% %TABLE 
% %________________________________________________________________________________

% \begin{table}[t]
%     \centering
%     \begin{tabular}{||c|c|c|c||}
%     \hline 
%         {Kernel}  & \thead{Lower \\Bound} & {GP-UCB} & {LP-GP-UCB }\\ \hline 
%         $\kse$ & $\Omega(\sqrt{n})$ &$\bm{\tilde{\mc{O}}(\sqrt{n})}$ & $\bm{\tilde{\mc{O}}(\sqrt{n})}$ \\[5pt] \hline 
%         %--------------------------------------------------------------------------------
%         $\kmat$ & $\Omega\big( n^{\frac{\nu+D}{2\nu+D}}\big)$  &\makecell{$\tilde{\mc{O}}\big( n^{\frac{2\nu + 3\tilde{D}}{4\nu + 2\tilde{D}}}\big)$ \\ \scriptsize{$\tilde{D}=D(D+1)$}} & $\bm{\tilde{\mc{O}}\lp n^{\frac{\nu+D}{2\nu+D}}\rp}$\\[5pt]  \hline 
%         %--------------------------------------------------------------------------------
%         $K \in \mc{K}$ & $\bigtimes$  &$\bigtimes$  & \makecell{$\tilde{\mc{O}}\big( n^{\frac{\alpha+D}{2\alpha+D}}\big)$\\ \scriptsize{$\alpha \in \{1/2, 1\}$}}\\[5pt] \hline 
%     \end{tabular}
%     \caption{Comparison of the bounds on $\creg$ obtained in this paper with the lower bounds of~\citep{scarlett2017lower} and the upper bounds on GP-UCB derived in~\citep{srinivas2012information}. The class of kernels $\mc{K}$ is defined in Prop.~\ref{prop:embed2}. In the table above, bold indicates that the upper bound matches the lower bound modulo polylog factors.}
%     \label{table:regret}
% \end{table}
% %________________________________________________________________________________
% %________________________________________________________________________________


%-------------------------------------------------------------------------------
% CONTEXTUAL BANDITS, SAFE BAYESIAN OPTIMIZATION, TIME-VARYING BAYEISIAN OPTIMIZATION
%-------------------------------------------------------------------------------
% \subsection{Extensions of GP bandits}
% \label{subsec:extensions}
% % \vspace{-0.5em}
% While we have mainly focused on the problem of GP bandits in this paper, the techniques developed can easily be extended to several related settings. In this section we discuss two such extensions. 

% \tbf{(i)} \emph{Parallel GP bandits:} This is a generalization of the purely sequential GP bandits, in which the unknown function $f$ can be evaluated in parallel in batches of a given size $m$. Prior work such as \citep{contal2013parallel} have shown that by combining the usual GP-UCB algorithm with a pure exploration scheme, we can achieve an improvement by a factor of $\sqrt{m}$ over the purely sequential GP-UCB algorithm. A similar modification can be employed to our LP-GP-UCB algorithm and thus we can also obtain the improved bounds on the simple regret for the parallel GP bandits as well. 

% % \tbf{(i)} Contextual GP bandits: This is the simplest generalization of the usual GP bandits, where at each time $t$ a \emph{context} $c_t \in \domain_c$ arrives, and the learner must select an action $a_t \in \domain_a$ and receive a reward $f(c_t, a_t)$. The goal is to select actions to minimize the contextual regret $\creg^c = \sum_{t=1}^n \max_{a \in \domain_a}f(a, c_t) - f(a_t, c_t)$. Under the assumption that $\f \in \rkhs$,   \citep{krause2011contextual} showed that this quantity can be upper bounded by $\tilde{\mc{O}}\lp \sqrt{n}\igain\rp$, where $\igain$ is now defined as a maximum over $\domain_c \times \domain_a$. Similar to the GP bandits case, this regret bound is loose for the \matern~family, and the techniques developed in this paper should be useful in obtaining improved regret bounds. The key technical task is to extend the  embedding result~(Prop.~\ref{prop:embed1}) to the case of \emph{composite kernels} over the product space $\domain_c \times \domain_a$, i.e., kernels formed by combining individual kernels $K_c$ and $K_a$ over the context and action spaces respectively~\citep[\S~5.1]{krause2011contextual}. 



% \tbf{(ii)} \emph{GP level set estimation:} In this problem, the goal is to estimate the $\tau-$level-set $S_\tau = \{x \in \domain\;:\; f(x) \geq \tau\}$ of an unknown function $\f$, for some $\tau \in \reals$. If an algorithm constructs an estimate of the level set $\hat{S}_\tau$, then the quality of reconstruction is measured by the uniform error $\mc{E}_n \coloneqq \sup_{x \in \hat{S}_\tau \Delta S_\tau}|f(x) -\tau|$. 
% For this problem, \citep{gotovos2013active} and \citep{bogunovic2016truncated} designed algorithms for which they showed that under the assumption that $\f \in \rkhs$ for some kernel $K$, we have $\mc{E}_n = \tilde{\mc{O}}\lp \igain/\sqrt{n}\rp$. This bound  is again loose for \matern~kernels. For this case as well, we can adapt the techniques developed in Section~\ref{sec:LPGPUCB} to design an algorithm and achieve improved performance. Informally, the major modification required is in the candidate point selection rule~(Line~\ref{algoline:candidate} of Alg.~\ref{algo:algo1}): instead of selecting a point with the largest UCB, we need to select points from cells with values close to $\tau$. 

% In addition to the above two problems, there are several other interesting cases in which our techniques may be beneficial, such as contextual GP bandits~\citep{krause2011contextual}, time-varying GP bandits~\citep{bogunovic2016time}, and adversarially robust GP bandits~\citep{bogunovic2018adversarially}.
% We leave the required derivations and modifications to extend our techniques to all these problems for future work. 
% % \vspace{-0.5em}
%-------------------------------------------------------------------------------
% PRACTICAL ISSUES
%-------------------------------------------------------------------------------
% \subsection{Practical Issues}
% \label{subsec:practical}
% % \vspace{-0.6em}
% While the LP-GP-UCB can achieve much tighter control over both simple and cumulative regret in comparison to the GP-UCB algorithm, we do not claim that these results can immediately translate into improved performance for practical problems. The reason is that some of the assumptions made, such as Assumption~\ref{assump:embed} and the condition that $n_E > \tilde{N}_k$, only kick in for very large values of $n$. Since most practical applications of GP bandits are in the small sample regime, it implies that the theoretical improvements may not be apparent in such cases. Furthermore, some steps of the LP-GP-UCB algorithm, such as the \maxerr~function, though mathematically well defined, may be computationally expensive to implement in practice.  

% Nevertheless, we can extract some practical design principles from LP-GP-UCB algorithm, which may be of practical utility: \\
% $\; \bullet \;$ Non-uniform partition of $\domain$: LP-GP-UCB maintains a partition of $\domain$ consisting of cells which allows it to  focus sampling in the near optimal parts of $\domain$. In practice, it might be more efficient to employ decision trees for constructing these partitions as they can learn the underlying structure in a more sample efficient manner. \\
% $\; \bullet \;$ Use of  local estimators: In LP-GP-UCB we used local polynomial estimators in candidate selection and cell expansion. In practice, depending on the application, other estimators such as projection estimators or kernel based estimators might also be useful. 
% % \vspace{-0.7em}



%________________________________________________________________________________
%________________________________________________________________________________
% \subsection{ Maximum Information Gain}
% \label{subsec:information_gain}
% % \vspace{-0.6em}
% In the analysis of the GP-UCB algorithm, \citep{srinivas2012information} first bound the instantaneous regret $\ireg(x_t) \coloneqq \f(x^*) - \f(x_t)$ with $\beta_t \sigma_t(x_t)$, and the proceed as follows:
% \begin{small}
% \begin{align}
% \label{eq:reg_analysis1}
%     \creg &
%     % = \sum_{t=1}^n \ireg(x_t)  
%     \leq \beta_n \sum_{t=1}^n \sigma_t  
%   \stackrel{(a)}{\leq} 
% \beta_n  \sqrt{ n \sum_{t=1}^n \sigma_t(x_t)^2 }   \nonumber  \\ 
% &    \stackrel{(b)}{\leq} \beta_n \sqrt{   n \;I(y_{[1:n]}, f)} 
%     \stackrel{(c)}{\leq} \beta_n\sqrt{ n \igain}. 
% \end{align}
% \end{small}
% The justification of these steps can be found in \citep{srinivas2012information}. For \matern~kernels, we know that this chain of inequalities results in a loose bound. However, it is not clear whether the looseness of the bounds is due to an inherent limitation of the GP-UCB algorithm, or a result of loose analysis.

% % \vspace{-0.4em}
% To empirically study this, we conducted a numerical experiment whose result is plotted in Figure~\ref{fig:fig1}. 
% In this experiment, we ran the GP-UCB algorithm with \matern~kernel ($\nu=2.5$) on a common benchmark function (Rosenbrock) over $\domain = [0,1]^4$ for $n=5000$ steps, and plotted $\log (\sum_{t=1}^n \sigma_t(x_t))$ (red) and $\log(\sqrt{n\igain})$ vs $\log n$ where we used the upper bound on $\igain$ derived in \citep{srinivas2012information}. The figure clearly shows that the growth of $\sum_t \sigma_t(x_t)$ is slower than $\sqrt{n\igain}$, which suggests that GP-UCB actually performs better compared to the bounds of \citep{srinivas2012information} for \matern~kernels. 

%  The smoothness results that we derived for \matern kernels in Prop.~\ref{prop:embed1} in combination with the ideas of \citep{lederer2019posterior} may be helpful in obtaining a tighter characterization of the posterior variances, thus resulting in improved bounds for the GP-UCB algorithm.
% % \vspace{-1.2em}
% %--------------------------------------------------------------------------------
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=3in, height=2in]{SECTIONS/fig.png}
% \caption{The blue line plots the theoretical bound on $\log(\sqrt{n\igain})$  derived by \citep{srinivas2012information} for \matern~kernel with $\nu=2.5$, while the red line shows the plot of the quantity $\log(\sum_{t=1}^n \sigma_t(x_t))$ for the GP-UCB algorithm. To compare the slope we shifted both lines to pass through $(0,0)$.}
%     \label{fig:fig1}
% \end{figure}
% %--------------------------------------------------------------------------------



==> Preliminaries.tex <==
% \vspace{-1em}
In this section, we recall several definitions which are required for presenting our results and fix some notations. 

A function $K: \domain \times \domain \mapsto \mbb{R}$ is called a positive-definite \emph{kernel} if for all $m \in \mbb{N}$ and $a_i \in \reals$ for $1 \leq i \leq m$, the following inequality holds: $\sum_{i=1}^m\sum_{j=1}^m a_i K(x_i, x_j) a_j \geq 0$. 
% Equivalently, this means that the $m \times m$ \emph{Gram matrix} $K_{XX} = [K(x_i,x_j)]_{1 \leq i,j\leq m}$ for any choice of $(x_i)_{i=1}^m \subset \domain$ and $m \in \mbb{N}$, is a positive-semidefinite matrix. 
Every kernel function, $K$,  can be used to define a collection of functions $\{K(\cdot, x): \domain \mapsto \reals, \; x \in \domain\}$ and the corresponding linear span  $\mc{G}_K \coloneqq \{ \sum_{i=1}^m a_i K(\cdot, x_i)\; : \; m \in \mbb{N}, \; (x_i)_{i=1}^m \subset \domain, (a_i)_{i=1}^m \subset \reals\}$.  Using the positive-definiteness of $K$, the following inner-product can be defined on $\mc{G}_K$, $\langle f, g \rangle_{K} = \sum_{i=1}^{m_1} \sum_{j=1}^{m_2}a_i  b_j K(x_i, z_j)$ for $f=\sum_{i=1}^{m_1} a_i K(\cdot, x_i)$ and $g=\sum_{j=1}^{m_2} b_j K(\cdot, z_j)$. Thus $\lp \mc{G}_K, \langle \cdot, \cdot \rangle_{K} \rp$ is an inner-product space, which may not be complete. 
The \emph{Reproducing Kernel Hilbert Space} associated with kernel $K$, denoted by $\rkhs$,  is defined as the completion of the inner product space $\lp \mc{G}_K, \langle \cdot, \cdot \rangle_{K} \rp$. 

Two of the most commonly used kernels in machine learning are the Squared-Exponential~(SE) kernel $\kse$ and the \matern family of kernels, $(\kmat)_{\nu>0}$, parameterized by a smoothness parameter $\nu$. For $x, z \in \domain$ such that $\|x-z\|=r$, they are defined as 
\begin{align*}
    &\kse(x, z) = \kse (r) = \exp \lp - \frac{ r^2}{2 \theta_l^2} \rp,  \qquad 
    \kmat(x, z) = \kmat (r) = \frac{2^{1-\nu}}{\Gamma(\nu)} \lp \frac{ \sqrt{2 \nu }r}{\theta_l} \rp^{\nu} J_\nu \lp \frac{ \sqrt{2 \nu }r}{\theta_l} \rp, 
\end{align*}
where $\Gamma(\cdot)$ is the Gamma function,  $J_{\nu}$ represents the modified Bessel's function of the second kind, and $\theta_l>0$ is the length-scale parameter. 
In addition to the above two kernels, some other important kernels used in applications are Rational-Quadratic kernels $\krq$, Gamma-exponential kernels $\kgexp$ and piece-wise polynomial kernels. A detailed description of these kernel functions can be found in \citep[Chapter~4]{williams2006gaussian}. 


For $0<\alpha\leq 1$, we use $\mc{C}^{0,\alpha}(\domain)$ to denote the the space of \holder~continuous functions $g:\domain \mapsto \mbb{R}$, which satisfy $[g]_\alpha < \infty$ where $[\cdot]_\alpha$ is defined in~\eqref{eq:holder}. Furthermore for $k \geq 1$, we can define higher order \holder~spaces $\mc{C}^{k,\alpha}$, as the collection of functions $g$ with $\|g\|_{\mc{C}^{k,\alpha}}<\infty$. In the definition of $\|\cdot\|_{\mc{C}^{k,\alpha}}$ in~\eqref{eq:holder},  we have $\|g\|_u \coloneqq \sup_{x\in \domain} |g(x)|$ and $\partial^a g$ denotes the derivative of $g$ with multi-index $a = (a_1, a_2, \ldots, a_D)\in\mbb{N}^D$ and $|a|\coloneqq \sum_{i=1}^Da_i$. 
\begin{align}
\label{eq:holder}
    [g]_\alpha \coloneqq \sup_{ x_1, x_2 \in \domain} \; \frac{ |g(x_1) - g(x_2)|}{\|x_1-x_2\|^\alpha}, \quad 
     \|g\|_{\mc{C}^{k,\alpha}} \coloneqq \sum_{|a|\leq k} \|\partial^ag\|_u +  \sum_{|a|=k} [\partial^ag]_{\alpha}.
\end{align}

% Now, let $\partial^a g$ denote the derivative of $g$ where $a = (a_1, a_2, \ldots, a_D)\in\mbb{N}^D$ is a multi-index.  Define $|a|=\sum_{i=1}^Da_i$ and $\|g\|_u = \sup_{x \in \domain}|g(x)|$ (the uniform or $\sup$ norm). 
%  Then we can define higher order \holder~spaces, $\mc{C}^{k,\alpha}$, as the collection of $g:\domain \mapsto \mbb{R}$ which satisfy


% Higher order \holder~spaces, $\mc{C}^{k,\alpha}(\domain)$ for $k \in \mbb{N}$, can be defined as the class of functions $g$ whose $k^{th}$ derivative belongs to $\mc{C}^{0, \alpha}$. 
% The corresponding functions space is $\holderspace \coloneqq \{ g \in \cont{\domain}\; : [g]_\alpha < \infty\}$ and the corresponding \holder ball as $\holderspace(L) \coloneqq \{ g \in \holderspace\; : \; [g]_\alpha \leq L\}$.

%--------------------------------------------------------------------------------
%NOTATIONS
%--------------------------------------------------------------------------------
\tbf{Notations.} We now describe the notations used in this paper. Recall that $f$ is the objective function mapping $\mc{X} = [0,1]^D$ to $\mc{Y} = \mbb{R}$. The function $f$ can be accessed through a noisy evaluations of the form $y = f(x) + \eta$, where the additive noise $\eta$ is assumed to be $\sigma$ sub-gaussian. We will use the term \emph{cell} to refer to subsets $E$ of $\domain$ of the form $E = \{x \in \domain \;:\; \|x - x_E\|_\infty \leq r_E/2\}$. The terms $x_E$ and $r_E$ shall be referred to as the \emph{center} and the \emph{side-length} of $E$. Given a cell $E$, a point $x\in E$ and a real number $h>0$, we use $E_{x,h}$ to denote the set $\{z \in E\;:\; \|z-x\|_\infty \leq h\}$.  Given a kernel function $K$, we shall use the term $\rkhs$ and $\|\cdot\|_K$ to denote the associated RKHS and the RKHS norm respectively. Also for any $x \in \domain$, we use $K_x(\cdot)$ to denote the feature map  $K(\cdot, x)$ associated with the point $x$. 
Let $\mc{D} = \{ (x_i, y_i) \; : \; 1 \leq i \leq m\} \subset \mc{X} \times \mc{Y}$ denote a labelled data set, and introduce $\mc{D}_\mc{X}\coloneqq \{x \; : \exists y \in \mc{Y}, (x, y) \in \mc{D}\}$ and $\mc{D}_\mc{Y} \coloneqq \{ y \;:\; \exists x \in \mc{X}, (x,y) \in \mc{D}\}$. For a cell $E \subset \mc{X}$, we use $\mc{D}^{(E)}$ to denote the subset of $\mc{D}$ with $x_i \in E$. The sets $\mc{D}_{\X}^{(E)}$ and $\mc{D}_{\mc{Y}}^{(E)}$ are also defined in an analogous manner. For  positive integers $k$ and $D$, we use $\mc{P}_D^k$ to denote the set of all polynomials in $D$ variables of degree $k$. Given a function $f:\domain \mapsto \mbb{R}$ and $E \subset \domain$, we define the quantity $\Phi_k(f, E) = \inf_{p \in \mc{P}_D^k}\sup_{x \in E} |f(x) - p(x)|$ as the smallest uniform approximation error of $f$ with a polynomial $p$ in $\mc{P}_D^k$. 
% \vspace{-1.4em}
